Point Tracking as a Temporal Cue for Robust Myocardial Segmentation in Echocardiography Videos

Purpose: Myocardium segmentation in echocardiography videos is a challenging task due to low contrast, noise, and anatomical variability. Traditional deep learning models either process frames independently, ignoring temporal information, or rely on memory-based feature propagation, which accumulates error over time. Methods: We propose Point-Seg, a transformer-based segmentation framework that integrates point tracking as a temporal cue to ensure stable and consistent segmentation of myocardium across frames. Our method leverages a point-tracking module trained on a synthetic echocardiography dataset to track key anatomical landmarks across video sequences. These tracked trajectories provide an explicit motion-aware signal that guides segmentation, reducing drift and eliminating the need for memory-based feature accumulation. Additionally, we incorporate a temporal smoothing loss to further enhance temporal consistency across frames. Results: We evaluate our approach on both public and private echocardiography datasets. Experimental results demonstrate that Point-Seg has statistically similar accuracy in terms of Dice to state-of-the-art segmentation models in high quality echo data, while it achieves better segmentation accuracy in lower quality echo with improved temporal stability. Furthermore, Point-Seg has the key advantage of pixel-level myocardium motion information as opposed to other segmentation methods. Such information is essential in the computation of other downstream tasks such as myocardial strain measurement and regional wall motion abnormality detection. Conclusion: Point-Seg demonstrates that point tracking can serve as an effective temporal cue for consistent video segmentation, offering a reliable and generalizable approach for myocardium segmentation in echocardiography videos. The code is available at https://github.com/DeepRCL/PointSeg.

==> sections/1_related_work.tex <==
\section{Related Work}

\subsection{Medical Image Segmentation}
Medical image segmentation has been widely studied, with UNet~\cite{unet} and SwinUNet~\cite{swinunet} achieving strong performance through hierarchical feature extraction. While effective for static images, these models lack temporal modeling, making them suboptimal for video-based tasks requiring motion consistency.

Recent adaptations of the Segment Anything Model (SAM)~\cite{sam}, such as MedSAM~\cite{medsam} and SAMUS~\cite{samus}, extend SAM to medical imaging but remain frame-independent, segmenting each frame in isolation. MedSAM2~\cite{medsam2} treats 3D segmentation as a video problem, leveraging a memory bank to model long-term dependencies. However, its design prioritizes volumetric consistency rather than real-time motion cues, limiting applicability to dynamic cardiac imaging.

\subsection{Video-based Segmentation}
MemSAM~\cite{memsam} introduces a space-time memory module to propagate contextual information across frames, improving segmentation stability. While effective for long-term consistency, memory-based approaches rely on feature aggregation from previous frames rather than explicit motion modeling, making them less responsive to rapid deformations such as myocardial contractions. They also struggle with temporal discontinuities, where accumulated errors propagate through time.

\subsection{Point Tracking as a Temporal Cue}
Point tracking provides a complementary motion-aware signal that can enhance dense prediction tasks such as segmentation. Unlike memory-based approaches, which rely on global feature aggregation, point tracking captures fine-grained correspondences between frames, making it a valuable temporal cue for segmenting dynamic structures.

In natural images, transformer-based tracking models~\cite{cotracker,taptrv2,tapir} learn dense point correspondences across frames, enabling robust motion estimation. However, these models are trained on synthetic datasets and struggle with domain shifts when applied to medical imaging, particularly ultrasound, which is characterized by speckle noise, varying contrast, and artifacts.

In echocardiography, EchoTracker~\cite{echotracker} employs a coarse-to-fine tracking strategy to follow tissue points throughout a cardiac cycle, achieving improved tracking accuracy over optical flow-based methods. However, such approaches rely on manually labeled datasets, which are limited in size and restrict generalization. The scarcity of labeled tracking data in echocardiography makes it difficult to train models that generalize across different imaging conditions.

Long-term point trajectories have also been explored as a supervisory signal for segmentation~\cite{lrtl}, leveraging motion consistency to group object points. While this suggests that tracking can aid segmentation, trajectory-based methods alone lack sufficient spatial context for dense predictions.

Despite these challenges, tracking-based motion estimation remains largely underexplored for segmentation. Since point tracking alone does not provide complete spatial information, an effective segmentation model must integrate both spatial and temporal cues while overcoming the limitations of small, manually annotated datasets.


==> sections/4_results.tex <==
\begin{table}[h!]
\caption{\textbf{Point tracking performance} on the synthetic dataset. 
The results are evaluated using Average Jaccard (AJ), Average Points Within Range ($<\delta_{avg}$), 
and Occlusion Accuracy (OA).}
\label{tab:tracking_results}
\centering
\begin{tabular*}{\textwidth}{@{\extracolsep\fill}llccc}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Training Data} & 
\multicolumn{3}{@{}c@{}}{SynUS (test)~\cite{synus}} \\
\cmidrule(lr){3-5}
 & & AJ$\uparrow$ & $<\delta_{avg}$$\uparrow$ & OA$\uparrow$ \\ 
\midrule
EchoTracker~\cite{echotracker} & Private Data & 0.762 & 0.831 & - \\
EchoTracker~\cite{echotracker} & Private Data + SynUS~\cite{synus} & 0.800 & 0.850 & 0.900 \\
TAPTR~\cite{taptrv2} & Kubric~\cite{kubric} & 0.695 & 0.834 & 0.894 \\
PointSeg (ours) & SynUS~\cite{synus} & \textbf{0.879} & \textbf{0.928} & \textbf{0.993} \\
\bottomrule
\end{tabular*}
\footnotetext{All metrics are reported on the SynUS synthetic dataset~\cite{synus}. 
Higher values indicate better performance.}
\end{table}



\begin{table}
    \centering
    \caption{\textbf{Segmentation performance} on CAMUS and the private dataset. Models are trained and tested on CAMUS, then fine-tuned and tested on private data for domain adaptation.}\label{tab:segmentation_results}
    \begin{adjustbox}{center,max width=\textwidth}
    \begin{tabular}{lcccccccc}
        \toprule
        \multirow{2}{*}{Method} & \multicolumn{4}{c}{CAMUS Dataset~\cite{camus}} & \multicolumn{4}{c}{Private Dataset} \\
        \cmidrule(lr){2-5}\cmidrule(lr){6-9}& mDice$\uparrow$ & HD95$\downarrow$ & mIoU$\uparrow$ & ASSD$\downarrow$ & mDice$\uparrow$ & HD95$\downarrow$ & mIoU$\uparrow$ & ASSD$\downarrow$ \\ 
        \midrule
        UNet~\cite{unet} & 0.835(0.606) & 4.877(2.313) & 0.721(0.084) & 1.982(0.633) & 0.698(0.105) & 5.122(4.318) & 0.546(0.117) & 1.982(1.277) \\
        SwinUNet~\cite{swinunet} & 0.855(0.055) & 4.154(1.690) & 0.750(0.079) & 1.686(0.592) & 0.709(0.094) & 4.796(2.557) & 0.557(0.106) & 1.938(0.830) \\
        \midrule
        MedSAM2~(click)~\cite{medsam2} & 0.795(0.065) & 6.386(2.708) & 0.665(0.086) & 2.416(0.796) & 0.632(0.124) & 6.301(4.442) & 0.473(0.123) & 2.313(1.169)\\
        MedSAM2~(bbox)~\cite{medsam2} & 0.856(0.051) & 4.055(1.508) & 0.758(0.070) & 1.689(0.651) & 0.616(0.222) & 6.937(6.870) & 0.476(0.200) & 2.435(2.136)\\
        MemSAM~\cite{memsam} & 0.850(0.065) & 5.922(6.988) & 0.744(0.092) & 2.074(1.254) & 0.695(0.111) & 6.497(6.190) & 0.543(0.125) & 2.368(1.180) \\
        EchoPTS (ours) & \textbf{0.864(0.050)} & \textbf{3.859(1.439)} & \textbf{0.764(0.073)} & \textbf{1.592(0.558)} & 0.683(0.114) & 5.017(2.805) & 0.529(0.125) & 2.062(1.030) \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
\end{table}

\begin{table}
    \centering
    \caption{\textbf{Generalization results} of EchoPTS and state-of-the-art methods, trained on the CAMUS~\cite{camus} dataset and evaluated on the private dataset. This evaluation assesses each model’s ability to generalize to unseen data.}\label{tab:generalization}
    \begin{adjustbox}{center,max width=\textwidth}
    \begin{tabular}{lcccc}
        \toprule
        \multirow{2}{*}{Method}  & \multicolumn{4}{c}{Private Dataset} \\
        \cmidrule(lr){2-5}& mDice$\uparrow$ & HD95$\downarrow$ & mIoU$\uparrow$ & ASSD$\downarrow$ \\ 
        \midrule
        UNet~\cite{unet} & 0.500(0.153) & 16.096(13.108) & 0.347(0.133) & 0.747(2.967) \\
        SwinUNet~\cite{swinunet} & 0.591(0.101) & 10.394(8.118) & 0.427(0.100) & 3.764(1.794) \\
        \midrule
        MedSAM2 (click)~\cite{medsam2} & 0.530(0.102)& 13.300(7.374)& 0.367(0.093)& 4.637(1.725)\\
        MedSAM2 (bbox)~\cite{medsam2} & 0.528(0.273)& \textcolor{red}{7.994(5.458)}& 0.399(0.219)& \textcolor{red}{2.907(1.405)}\\
        MemSAM~\cite{memsam} & 0.594(0.122) & 11.837(9.851) & 0.433(0.121) & 4.428(2.406) \\
        EchoPTS (ours) & \textbf{0.603(0.111)} & \textbf{8.130(2.981)} & \textbf{0.440(0.111)} & \textbf{3.379(1.105)} \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
\end{table}

